Spacetime Meshing for Discontinuous Galerkin Methods

Spacetime discontinuous Galerkin (SDG) finite element methods are used to solve such PDEs involving space and time variables arising from wave propagation phenomena in important applications in science and engineering. To support an accurate and efficient solution procedure using SDG methods and to exploit the flexibility of these methods, we give a meshing algorithm to construct an unstructured simplicial spacetime mesh over an arbitrary simplicial space domain. Our algorithm is the first spacetime meshing algorithm suitable for efficient solution of nonlinear phenomena in anisotropic media using novel discontinuous Galerkin finite element methods for implicit solutions directly in spacetime. Given a triangulated d-dimensional Euclidean space domain M (a simplicial complex) and initial conditions of the underlying hyperbolic spacetime PDE, we construct an unstructured simplicial mesh of the (d+1)-dimensional spacetime domain M x [0,infinity). Our algorithm uses a near-optimal number of spacetime elements, each with bounded temporal aspect ratio for any finite prefix M x [0,T] of spacetime. Our algorithm is an advancing front procedure that constructs the spacetime mesh incrementally, an extension of the Tent Pitcher algorithm of Ungor and Sheffer (2000). In 2DxTime, our algorithm simultaneously adapts the size and shape of spacetime tetrahedra to a spacetime error indicator. We are able to incorporate more general front modification operations, such as edge flips and limited mesh smoothing. Our algorithm represents recent progress towards a meshing algorithm in 2DxTime to track moving domain boundaries and other singular surfaces such as shock fronts.

==> short-abstract.tex <==
Important applications in science and engineering, such as modeling
traffic flow, seismic waves, electromagnetics, and the simulation of
mechanical stresses in materials, require the high-fidelity numerical
solution of hyperbolic partial differential equations (PDEs) in space
and time variables.  Spacetime discontinuous Galerkin (SDG) finite
element methods are used to solve such PDEs arising from wave
propagation phenomena.

To support an accurate and efficient solution procedure using SDG
methods and to exploit the flexibility of these methods, we give a
meshing algorithm to construct an unstructured simplicial spacetime
mesh over an arbitrary simplicial space domain.  Our algorithm is the
first adaptive spacetime meshing algorithm suitable for efficient
solution of nonlinear phenomena using spacetime discontinuous Galerkin
finite element methods.  Given a triangulated $d$-dimensional
Euclidean space domain $\sp$ (a simplicial complex) corresponding to
time $t=0$ and initial conditions of the underlying hyperbolic
spacetime PDE, we construct an unstructured simplicial mesh of the
$(d+1)$-dimensional spacetime domain $\spt$.  Our algorithm uses a
near-optimal number of spacetime elements, each with bounded temporal
aspect ratio for any finite prefix of $\spt$.  When $d \le 2$, our
algorithm varies the size of spacetime elements to an
\aposteriori{} numerical estimate.  Certain facets of our mesh satisfy
gradient constraints that allow interleaving mesh generation with the
SDG solver.  Our meshing algorithm thus supports an efficient
parallelizable solution strategy by SDG methods.

